Indoor Geometry Generator (IGG) Manual

The Indoor Geometry Generator (IGG) is able to generate automatically simplified indoor geometry and its associated unstructured mesh for Computational Fluid Dynamics (CFD) simulations purposes given very simple user inputs. A large number of indoor features are supported by IGG such as (non-exhaustive list): shelves, tills, tables, chairs, seats... Smaller features such as laptops, computer towers and screens can also be included. In addition, doors/windows as well as ventilation inlet and outlet can be taken into account. Finally, the adding of simplified shape of humans standing, sitting or lying are also supported by IGG. IGG allows the user to generate without much effort indoor geometries such that shop, train, bus, plane, school, open spaces..., while being fully consistent with CFD requirements. The geometry and the mesh are outputted in GMSH format supported by both Fluidity and IC-FERST open-source finite-element CFD software.

==> BackUp.tex <==
Algorithm
\begin{enumerate}
    \item Read input files and generate the initial polygons: Polygon\_Initialisation()
    \item Add points to features when they are touched by another features
    \begin{itemize}
        \item Add points coming from the other feature
        \item Add points on the other surfaces of this feature
        \item ...
    \end{itemize}
    \item ...
\end{enumerate}
